Simulating Weighted Automata over Sequences and Trees with Transformers

Transformers are ubiquitous models in the natural language processing (NLP) community and have shown impressive empirical successes in the past few years. However, little is understood about how they reason and the limits of their computational capabilities. These models do not process data sequentially, and yet outperform sequential neural models such as RNNs. Recent work has shown that these models can compactly simulate the sequential reasoning abilities of deterministic finite automata (DFAs). This leads to the following question: can transformers simulate the reasoning of more complex finite state machines? In this work, we show that transformers can simulate weighted finite automata (WFAs), a class of models which subsumes DFAs, as well as weighted tree automata (WTA), a generalization of weighted automata to tree structured inputs. We prove these claims formally and provide upper bounds on the sizes of the transformer models needed as a function of the number of states the target automata. Empirically, we perform synthetic experiments showing that transformers are able to learn these compact solutions via standard gradient-based training.

==> macros.tex <==
\usepackage{mathtools}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\newcommand{\frec}{\phi} 
\newcommand{\fout}{\psi}

\newcommand{\depth}{\mathrm{depth}}
\let\vecarrow\vec
 \usepackage{relsize}
\newcommand{\vvf}{{\vecarrow{f}}}

\usepackage{etoolbox}
\usepackage{xparse}

%% Hacks
\renewcommand{\enspace}{}
\newcommand{\R}{\Rbb}
\newcommand{\e}{\ten}
%\renewcommand{\hat}{\widehat}
\newcommand{\bmat}[1]{\left[\begin{matrix}
#1
\end{matrix}\right]}

\newcommand{\comment}[1]{{\color{OliveGreen}[#1]}}

\newcommand{\hatskew}[1]{\skew{4}\hat{#1}}
\let\oldv\v

%% Macros to make visible comments while writing the paper

%\newcommand{\comment}[1]{}



%% Probability notations
\newcommand{\Prob}{\mathbb{P}}
\DeclareMathOperator*{\Esp}{\mathbb{E}}
%\newcommand{\Esp}{\mathbb{E}}
\newcommand{\Var}{\mathbb{V}}

%% Vectors, matrices and tensors
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\vecs}[1]{\ensuremath{\mathbf{\boldsymbol{#1}}}}
\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mats}[1]{\ensuremath{\mathbf{\boldsymbol{#1}}}}
\newcommand{\ten}[1]{\mat{\ensuremath{\boldsymbol{\mathcal{#1}}}}}

%% Tensor operations
% tensor times matrix
\newcommand{\ttm}[1]{\times_{#1}}
% tensor times vector
\newcommand{\ttv}[1]{\bullet_{#1}}
% matricisation
%\newcommand{\tenmat}[2]{\mat{#1}_{(#2)}}
\newcommand{\tenmat}[2]{\ten{#1}_{(#2)}}
\newcommand{\tenmatpar}[2]{(#1)_{(#2)}}
\newcommand{\tenmatgen}[2]{{(#1)}_{\langle\!\langle #2\rangle\!\rangle}}
% Generalized Trace
%\newcommand{\gentrace}[2]{\Tr[#1]_{#2}}
\newcommand{\gentrace}[2]{\langle\!\langle #1\rangle\!\rangle_{#2}}
\newcommand{\TT}[1]{\llbracket #1 \rrbracket}


% sample number
\newcommand{\nsample}[1]{^{(#1)}}

\usepackage{pgffor}

% % all mathbb letters, e.g. \Rbb -> \mathbb{R}

\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x bb\endcsname{\noexpand\ensuremath{\noexpand\mathbb{\x}}}
}

% all mathcal letters, e.g. \Acal -> \mathcal{A}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x cal\endcsname{\noexpand\ensuremath{\noexpand\mathcal{\x}}}
}

% all tensor letters, e.g. \At -> \ten{A}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x t\endcsname{\noexpand\ensuremath{\noexpand\ten{\x}}}
}

% all matrices letters, e.g. \Ab -> \mat{A}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x b\endcsname{\noexpand\ensuremath{\noexpand\mat{\x}}}
}

%all matrices letters, e.g. \vb -> \vec{v}
% defining \sb messes with the \url command...
\foreach \x in {a,...,r}{%
\expandafter\xdef\csname \x b\endcsname{\noexpand\ensuremath{\noexpand\vec{\x}}}
}
\foreach \x in {t,...,z}{%
\expandafter\xdef\csname \x b\endcsname{\noexpand\ensuremath{\noexpand\vec{\x}}}
}

% all texttt digits, e.g. \t1 -> \texttt{1}
%\foreach \x in {0,...,9}{%
%t\expandafter\xdef\csname \x \endcsname{\noexpand\ensuremath{\noexpand\texttt{\x}}}
%}


% common matrices and tensors
\newcommand{\A}{\mat{A}}
\newcommand{\B}{\mat{B}}
\newcommand{\C}{\mat{C}}
\newcommand{\Hten}{\ten{H}}
\newcommand{\T}{\ten{T}}
\newcommand{\W}{\ten{W}}
\newcommand{\G}{\ten{G}}
\newcommand{\Y}{\ten{Y}}
\newcommand{\U}{\mat{U}}
\renewcommand{\H}{\mat{H}}
\newcommand{\Q}{\mat{Q}}
\newcommand{\X}{\mat{X}}
\newcommand{\I}{\mat{I}}
\newcommand{\E}{\mat{E}}
\newcommand{\M}{\mat{M}}
\newcommand{\K}{\mat{K}}
\newcommand{\D}{\mat{D}}
\newcommand{\V}{\mat{V}}
\renewcommand{\P}{\mat{P}}
\renewcommand{\S}{\mat{S}}
\renewcommand{\v}{\vec{v}}
\renewcommand{\u}{\vec{u}}
\newcommand{\x}{\vec{x}}
% adding a tilde for input matrix and output tensor
\newcommand{\tX}{\tilde{\X}}
\newcommand{\tY}{\tilde{\Y}}
\newcommand{\y}{\vec{y}}
\newcommand{\Proj}{\mats{\Pi}}

\newcommand{\Pref}{P}
\newcommand{\Suff}{S}

%% Math environments
\newtheorem*{theorem*}{Theorem}
\newtheorem*{corollary*}{Corollary}%
\newtheorem*{proposition*}{Proposition}%
\ifcsdef{theorem}{}{
\newtheorem{theorem}{Theorem}%
\newtheorem{proposition}{Proposition}%
\newtheorem{lemma}{Lemma}%
\newtheorem{definition}{Definition}%
\newtheorem{corollary}[theorem]{Corollary}%
\newtheorem{condition}{Condition}%
\newtheorem{claim}{Claim}%
\newtheorem{remark}{Remark}%
\newtheorem{example}{Example}%
}
\newtheorem{pbm}{Problem}%
\newtheorem*{pbm*}{Problem}%
\newtheorem{algo}{Algorithm}%
\newtheorem*{algo*}{Algorithm}%

%% Products
\newcommand{\kron}{\otimes}
\newcommand{\krao}{\odot}
\newcommand{\hadam}{*}
\newcommand{\outprod}{\circ}
\newcommand{\dirsum}{\oplus}

%% Miscellaneous math stuff
\DeclareMathOperator*{\Tr}{Tr} %trace
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\vectorize}[1]{\mathrm{vec}(#1)}
\DeclareMathOperator*{\reshape}{reshape}
\newcommand{\eqdef}{\triangleq}
\newcommand{\vtimes}[1]{\ \overline{\times}_{#1}\ }
\DeclareMathOperator*{\rank}{rank}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\Ker}{\mathrm{Ker}}
\renewcommand{\Im}{\mathrm{Im}}
\newcommand{\bigo}[1]{\mathcal{O}\left(#1\right)}
\newcommand{\singv}{\mathfrak{s}}
\newcommand{\singvmin}[1]{\singv_{\min}(#1)}
\newcommand{\vspan}[1]{span(#1)}
\newcommand{\dotprod}[2]{\langle #1, #2\rangle}

\newcommand{\pinv}{^\dagger}
\newcommand{\inv}{^{-1}}
\newcommand{\invtop}{^{-\top}}

\newcommand{\res}[1]{\overline{#1\rule{0pt}{1.7mm}}}



%%% WA / WTA
\newcommand{\nstates}{n}

% String automata
\newcommand{\szerosymbol}{\alpha}
\newcommand{\szero}{\vecs{\szerosymbol}}

\newcommand{\sinfsymbol}{\omega}
\newcommand{\sinf}{\vecs{\sinfsymbol}}

\DeclareDocumentCommand{\wa}{  O{A} O{\szero} O{\sinf} }%
{(#2,\{\mat{#1}^\sigma\}_{\sigma\in\Sigma},#3)}
\DeclareDocumentCommand{\waR}{  O{A} O{\Rbb^\nstates} O{\szero} O{\sinf} }%
{(#2,#3,\{\mat{#1}^\sigma\}_{\sigma\in\Sigma},#4)}

\newcommand{\wai}[1]{(\szero_{#1},\{\mat{A}_{#1}^\sigma\}_{\sigma\in\Sigma},\sinf_{#1})}

\newcommand{\vvszerosymbol}{\Alpha}
\newcommand{\vvszero}{\vecs{\vvszerosymbol}_0}
\newcommand{\vvsinfsymbol}{\Omega}
\newcommand{\vvsinf}{\mats{\vvsinfsymbol}}
\DeclareDocumentCommand{\vvwa}{  O{A} O{\szero} O{\vvsinf} }%
{(#2,\{\mat{#1}^\sigma\}_{\sigma\in\Sigma},#3)}

\newcommand{\vvwai}[1]{(\szero_{#1},\{\mat{A}_{#1}^\sigma\}_{\sigma\in\Sigma},\vvsinf_{#1})}


%\newcommand{\cev}[1]{\reflectbox{\ensuremath{\vecarrow{\reflectbox{\ensuremath{#1}}}}}}
\newcommand{\mirror}[1]{\widetilde{#1}}

% Tree automata
\newcommand{\tzerosymbol}{\alpha}
\newcommand{\tzero}{\vecs{\tzerosymbol}}

\newcommand{\tinfsymbol}{\omega}
\newcommand{\tinf}{\vecs{\tinfsymbol}}

\newcommand{\winf}{\tinf}  % shorcuts from the aistats paper
\newcommand{\wzero}{\tzero}

\DeclareDocumentCommand{\wta}{ O{T} O{\Rbb^\nstates} O{\tzero} O{\tinf} O{\Fcal}}%
{(#2,#3,\{\ten{#1}^g\}_{g\in #5_{\geq 1}},\{#4^\sigma\}_{\sigma\in #5_0})}

\newcommand{\wtaQ}{(\Rbb^\nstates , \Q^\top \tzero , 
\{\ten{A}^g(\Q^{-\top},\Q,\cdots,\Q)\}_{g\in\Fcal_{\geq 1}},
\{\Q^{-1}\tinf^\sigma\}_{\sigma\in\Fcal_0})}

\DeclareDocumentCommand{\trees}{g}{\IfNoValueTF{#1}{\mathfrak{T}}{\mathfrak{T}_{#1}}}
\DeclareDocumentCommand{\contexts}{g}{\IfNoValueTF{#1}{\mathfrak{C}}{\mathfrak{C}_{#1}}}
%\DeclareDocumentCommand{\contexts}{O{ }}{\mathfrak{C}_{#1}}

\newcommand{\Ts}{\trees{}}
\newcommand{\Cs}{\contexts{}}
\newcommand{\TF}{\Ts}
\newcommand{\CF}{\Cs}
\newcommand{\depth}[1]{\mathrm{depth}(#1)}
\newcommand{\size}[1]{\mathrm{size}(#1)}
\newcommand{\drop}[1]{\mathrm{drop}(#1)}
\newcommand{\yield}[1]{\langle #1 \rangle}
\newcommand{\sstar}{\Sigma^\star}
\newcommand{\gap}{\ast}
\newcommand{\ctm}{\mats{\Xi}}
\newcommand{\weight}{\mathrm{weight}}
\newcommand{\ltwot}{\ell^2_{\Ts}}
\newcommand{\ltwoc}{\ell^2_{\Cs}}

\newcommand{\gramc}{\mat{G}_{\contexts}}
\newcommand{\gramcapprox}{\hat{\mat{G}}_{\contexts}}
\newcommand{\gramt}{\mat{G}_{\trees}}
\newcommand{\gramtapprox}{\hat{\mat{G}}_{\trees}}


%%% GWM
\newcommand{\mapGMidsymbol}{\Gamma}
\newcommand{\mapGMid}[2]{\mapGMidsymbol_{id}(#1,#2)}

\newcommand{\ports}[1]{P(#1)}
\newcommand{\graphs}[1]{\mathfrak{G}_{#1}}
\newcommand{\ralph}{(\Sigma,\sharp)}
\newcommand{\singleton}[1]{G^{#1}}
\newcommand{\circstring}[1]{circ(#1)}
\newcommand{\stringgraph}[1]{graph(#1)}
\newcommand{\treegraph}[1]{graph(#1)}
\newcommand{\picgraph}[1]{graph(#1)}
\newcommand{\gwmprod}{\diamond}

\DeclareDocumentCommand{\gwm}{  O{M} O{\Fbb^\nstates}}{(#2, \{\ten{#1}^x\}_{x\in\Sigma})}
\DeclareDocumentCommand{\gwmcirc}{  O{M} O{\Rbb^\nstates}}{(#2, \{\mat{#1}^\sigma\}_{\sigma\in\Sigma})}
\DeclareDocumentCommand{\dgwm}{ O{M} O{\Fbb^\nstates}}{(#2, \{\ten{#1}^x\}_{x\in\Sigma},\gwmprod)}



\newcommand{\treemap}{\omega}
\newcommand{\graphmap}{\mu}

%%% Tensor-Valued Regression
\newcommand{\mlrank}[1]{\mathrm{rank}_{ml}(#1)}
\newcommand{\cprank}[1]{\mathrm{rank}_{CP}(#1)}

%% Tweaks
\renewcommand{\widehat}{\hat}















%% Mathematical sets with names
% all mathbb letters, e.g. \Rbb -> \mathbb{R}
\usepackage{pgffor}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x bb\endcsname{\noexpand\ensuremath{\noexpand\mathbb{\x}}}
}

% all mathcal letters, e.g. \Acal -> \mathcal{A}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x cal\endcsname{\noexpand\ensuremath{\noexpand\mathcal{\x}}}
}

% all tensor variables, e.g. \Aten -> \ten{A}
\usepackage{pgffor}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x ten\endcsname{\noexpand\ensuremath{\noexpand\ten{\x}}}
}

% all matrix variables, e.g. \Amat -> \mat{A}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x mat\endcsname{\noexpand\ensuremath{\noexpand\mat{\x}}}
}

% all vector variables, e.g. \avec -> \vec{a}
\foreach \x in {A,...,Z}{%
\expandafter\xdef\csname \x vec\endcsname{\noexpand\ensuremath{\noexpand\mat{\x}}}
}






\newcommand{\h}{\vec{h}}
\newcommand{\ie}{i.e.\ }
\newcommand{\eg}{e.g.\ }
\renewcommand{\e}{\vec{e}}
\newcommand{\xni}[2]{\x^{(#1)}_{#2}}
\usepackage[symbol]{footmisc}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
    % \usepackage{todonotes}
% \newcommand{\guillaume}[1]{\todo[inline,color=blue!40,caption={}]{{\it Guillaume:~}#1}}
% \newcommand{\tianyu}[1]{\todo[inline,color=green!40,caption={}]{{\it Tianyu:~}#1}}

